On the Origin of Linearity and Unitarity in Quantum Theory

We reconstruct the transformations of quantum theory using a physically motivated postulate. This postulate states that transformations should be locally applicable, and recovers the linear isometries from pure quantum theory, as well as the completely positive, trace-preserving maps from mixed quantum theory. Notably, in the pure case, linearity with respect to the superposition rule and reversibility are both derived from this locality principle.

==> oee.tex <==
\begin{proof} Clearly $\mathscr{L}_X$ maps normalized vectors to normalized vectors for all $X$. Now let us check that each part of local applicability holds for $\mathscr{L}^U$, beginning with state locality. For any $\ket{\psi} \in S_{A \otimes X}$ and $\ket{\phi} \in S_{X'}$:
\begin{align*}
    \mathscr{L}^{U}_{XX'}(\ket{\psi} \otimes \ket{\phi})  & =   (U \otimes I_{XX'}) \ket{\psi} \otimes \ket{\phi} \\
    & = (U \otimes I_{X}) \ket{\psi} \otimes \ket{\phi} \\
    & = \mathscr{L}^U_{X}(\ket{\psi}) \otimes \ket{\phi}.
\end{align*} Second, for compatibility with probabilities of measurements we have 
\begin{align*}
\mathscr{L}^U_X (\ket{\psi})^\dag  I \otimes \pi \ket{\mathscr{L}^U_X \psi} & =  \bra{\psi} (U^{\dagger} \otimes I) (I \otimes \pi) (U \otimes I) \ket{\psi} \\
 & = \bra{\psi} (I \otimes \pi)  (U^{\dagger} \otimes I) (U \otimes I) \ket{\psi} \\
 & = \bra{\psi}  I \otimes \pi \ket{\psi}
\end{align*} Finally, we need to check compatibility with the update rule, indeed note that 
\begin{align*}
 \frac{I \otimes \pi \ket{\mathscr{L}^U_X (\psi)}}{\sqrt{p(\psi, I \otimes \pi)}} & = \frac{(I \otimes \pi) (U \otimes I) \ket{\psi}}{\sqrt{p(\psi, I \otimes \pi)}} \\
  & = \frac{(U \otimes I) (I \otimes \pi) \ket{\psi}}{\sqrt{p(\psi, I \otimes \pi)}} \\
  & = \mathscr{L}^U_{X}  \Bigg(\frac{ I \otimes \pi \ket{\psi} }{\sqrt{p(\psi, I \otimes \pi)}} \Bigg).
 \end{align*} This completes the proof. 
\end{proof}
